Multi-IRS-assisted Multi-Cell Uplink MIMO Communications under Imperfect CSI: A Deep Reinforcement Learning Approach

Applications of intelligent reflecting surfaces (IRSs) in wireless networks have attracted significant attention recently. Most of the relevant literature is focused on the single cell setting where a single IRS is deployed and perfect channel state information (CSI) is assumed. In this work, we develop a novel methodology for multi-IRS-assisted multi-cell networks in the uplink. We consider the scenario in which (i) channels are dynamic and (ii) only partial CSI is available at each base station (BS); specifically, scalar effective channel powers from only a subset of user equipments (UE). We formulate the sum-rate maximization problem aiming to jointly optimize the IRS reflect beamformers, BS combiners, and UE transmit powers. In casting this as a sequential decision making problem, we propose a multi-agent deep reinforcement learning algorithm to solve it, where each BS acts as an independent agent in charge of tuning the local UE transmit powers, the local IRS reflect beamformer, and its combiners. We introduce an efficient information-sharing scheme that requires limited information exchange among neighboring BSs to cope with the non-stationarity caused by the coupling of actions taken by multiple BSs. Our numerical results show that our method obtains substantial improvement in average data rate compared to baseline approaches, e.g., fixed UE transmit power and maximum ratio combining.

==> protocol.tex <==
\section{Uplink Data Transmission Framework}
\label{sec:protocol}

\subsection{Observations at BS}

It would be critical to discuss available information to solve the optimization problem because conventional optimization methods cannot be used. 
Note that under dynamic environment in multiple IRS-aided multi-cell multi-user system, perfect channel estimation is challenging within the coherence time. 
Instead of all of the channels, 
BS can observe scalar effective channels as available information, which can be easily acquired in real-time.

When UE $(i,j)$ transmits pilot symbol with power ${p}_{i,j}[t]$, 
BS $\ell$ can measure the scalar effective channel $\hat {h}_{(i,j),\ell,k}[t] \in \mathbb{C}$ with the combiner ${\bf z}_{\ell, k}[t]$, given by
\begin{equation}
    \hat {h}_{(i,j),\ell,k}[t] = {\bf z}_{\ell, k}^H[t] \hat {\bf h}_{(i,j),\ell}[t],
\end{equation}
where $\hat {\bf h}_{(i,j),\ell}[t] \in \mathbb{C}^{N_T \times 1}$ is the effective channel from UE $(i,j)$ to BS $l$, given by
\begin{multline}
    \hat {\bf h}_{(i,j),\ell}[t] = \sqrt{p_{i,j}[t]} \bigg( {\bf h}^{\rm BS}_{ (i,j),\ell}[t]
    %\nonumber
     + \sum_{r=1}^L{\bf G}^{\rm BS}_{r,\ell} {\bf \Phi}_r[t] {\bf h}^{\rm IRS}_{ (i,j),r}[t] 
%    + {\bf g}^{\rm IRS }_{\ell}[t]
    \\
    + \sum_{r_2=1}^L \sum_{r_1=1}^L  {\bf G}^{\rm BS}_{r_2,\ell} {\bf \Phi}_{r_2}[t] {\bf G}^{\rm IRS}_{r_1,r_2} {\bf \Phi}_{r_1}[t] {\bf h}^{\rm IRS}_{ (i,j),r_1}[t] 
    \bigg).
\end{multline}
Here, the IRS beamformers are set to ${\bf \Phi}_r[t] = {\rm diag}({\boldsymbol \phi}_{r}[t])$ $\forall r$.


%It is reasonable to assume that BS $\ell$ obtains the effective channels $\hat {h}_{(i,j),\ell,k}[t] \; \forall i,j,k$ at time $t$ because pilot overhead for estimating the effective channels is negligible.

In small-scale networks, BS $\ell$ could obtain all of the scalar effective channels from all of the users $\forall(i,j)$ over the network with small pilot overhead, where $i \in \mathcal{L}$ and  $j \in \mathcal{K}$.
However, in large-scale networks, it would be burdensome to estimate all of the scalar channel estimates. 
Especially, in dynamic environment, it is not encouraged to estimate all of the scalar effective channels because real-time acquisition of the channel information is significant.
Therefore, we consider that BS $\ell$ obtains the effective channels from local UEs $(\ell, k)$ for $k \in \mathcal{K}$ and from UEs $(i,j)$ in neighboring cells, where $i \in \mathcal{B}_{\ell, \rm from}[t]$ and $j \in \mathcal{K}$.
The $\mathcal{B}_{\ell, \rm from}[t]$ is the set of indices of neighbouring cells in which UEs are interfering with the cell $\ell$, given by
\begin{multline}
    \mathcal{B}_{\ell, \rm from}[t] = \{ i \in \mathcal{L} : \sum_{j=1}^K \| \hat {\bf h}_{(i,j),\ell}[t] \|_2^2 \ge  \sum_{j=1}^K \| \hat {\bf h}_{(i',j),\ell}[t] \|_2^2 ,
    \\ |\mathcal{B}_{\ell, \rm from}[t]|=N_N, i \in \mathcal{B}_{\ell, \rm from}[t], i' \in \mathcal{L}\backslash \mathcal{B}_{\ell, \rm from}[t]   \},
\end{multline}
where $N_N$ is the number of neighbouring cells. In this paper, each cell is assumed to have two neighbouring cells, $N_N =2$.
%which are determined the sum of effective channel norm over UEs. 
The $\mathcal{B}_{\ell, \rm from}[t]$ is the set composed of $N_N$ indices corresponding $N_N$ largest elements, where each element is the sum of the square of effective channel norm over UEs. 
This implies that cell $\ell$ defines its neighbouring cells based on the interferences of  UEs in neighbouring cell $i \ne \ell$ to the BS $\ell$.
The norm estimation of the effective channel 
can be acquired by the antenna circuit before digital processing, for example, the automatic gain control (AGC) circuit \cite{mo2017channel}. 
Since the channel norm estimation does not require explicit values of effective channel, the set $\mathcal{B}_{\ell, \rm from}[t]$ can be determined in real-time. However, when the channels are correlated over time or slowly-varying, the set $\mathcal{B}_{\ell, \rm from}[t]$ will not change too much over time and does not need to be determined at every time constant.


%The BS $\ell$ can observe the effective 
%$\hat {h}_{(i,j),\ell,k}[t] $ from all local UEs and some neighbouring UEs.
%We denote the set of all local and neighbouring UEs corresponding to BS $\ell$ as $\mathcal{B}_{\ell}[t]$.
%The UEs close to BS $\ell$ are more likely to interfere with the data link of BS $\ell$ than distant UEs due to the effect of path loss.
%Therefore, the elements of 
%$\mathcal{B}_{\ell}[t]$ is selected based on BS-UE distance, 
%\begin{equation}
%    \mathcal{B}_{\ell}[t] = \{ (i,j): d_{\ell,(i,j)}[t] < \delta_{\ell}[t], i \in \mathcal{L}, j \in \mathcal{K} \}
%    \label{eq:Bl}
%\end{equation}
%where $d_{\ell,(i,j)}[t]$ is the distance between BS $\ell$ and UE $(i,j)$ and $\delta_{\ell}[t]$ is the distance threshold that can adaptively adjusted over time.



%it would be enough to estimate the scalar channels from neighbors.
%
%This set can be varying over time based on user mobility
%$k \in \mathcal{K}$ in cell $\ell$
%where $\mathcal{B}_{\ell}$ denotes the set of neighbouring users that interferes with the data links of BS $\ell$.
%BS $\ell$ obtains the scalar effective channels at  time $t$ because t
%Rhe pilot overhead for estimating the scalar effective channels is negligible, .

%BS $\ell$ obtains the scalar effective channels $\hat {h}_{(i,j),\ell,k}[t] $ for $(i,j) \in \mathcal{B}_{\ell}[t]$.
%From the scalar effective channels, 
BS can measure the received signal strength indicator (RSSI), which is the total power including the main signal, interferences signals over all UEs, and even the thermal noise.
BS can also obtain the reference signal received power (RSRP), which is the power of the specific main signal. These are the conventional measures to evaluate the signal quality in LTE standard \cite{LTEstandard}.
From RSSI and RSRP, BS can calculate signal-to-noise ratio (SINR). 
The SINR of UE $(\ell,k)$ for $ k \in \mathcal{K}$ can be formulated with scalar effective channels as
\begin{equation}
    {\hat {\rm SINR}}_{\ell, k}[t] =
{
\frac{ |\hat {h}_{(\ell,k),\ell,k}[t]|^2 }
{ \sum_{(i,j) \ne (\ell,k) } |\hat {h}_{(i,j),\ell,k}[t]|^2  + \sigma^2 }
}.
\end{equation}
Furthermore, from SINRs, BS $\ell$ can calculate the maximum achievable data rate of UE $(\ell,k)$ as
\begin{equation}
    {\hat R}_{\ell, k}[t] = W
{
\log_2 (1+ {\hat {\rm SINR}}_{\ell, k}[t])
}.
\end{equation}
where $W$ is the bandwidth.


%To obtain SINR, BS $\ell$ applies the designed combiner ${\bf z}_{\ell, k}[\tau]$ to the received effective channels $\hat {\bf h}_{(i,j),\ell}[\tau] \; \forall i,j$ and obtains $\hat {\rm SINR}_{\ell, k}[\tau] $ as
%\begin{equation}
%    {\hat {\rm SINR}}_{\ell, k}[\tau] =
%{
%\frac{ |{\bf z}_{\ell, k}^H[\tau] \hat {\bf h}_{(\ell,k),\ell}[\tau]|^2 }
%{ \sum_{(i,j) \ne (\ell, k)} |{\bf z}_{\ell, k}^H[\tau] \hat {\bf h}_{(i,j),\ell}[\tau]|^2  + \sigma^2 }
%}.
%\end{equation}

%As above, BS $\ell$ can acquire the effective channels from all users, $\{ \hat {\bf h}_{(i,j),\ell}[\tau] \}_{i,j}$, and SINRs of the local users in cell $\ell$, $\{ {\hat {\rm SINR}}_{\ell, k}[\tau] \}_{k} $.



%When UE $(i,j)$ transmits pilot symbol with power ${p}_{i,j}[\tau]$ at a given time $\tau$, 
%BS $\ell$ can measure the received effective channel $\hat {h}_{(i,j),\ell,k}[\tau]$, given by
%\begin{align}
%    & \hat {\bf h}_{(i,j),\ell}[\tau] = \sqrt{p_{i,j}[\tau]} \bigg( {\bf h}^{\rm BS}_{ (i,j),\ell}[\tau] + \sum_{r=1}^L{\bf G}^{\rm BS}_{r,\ell} {\bf \Phi}_r[\tau] {\bf h}^{\rm IRS}_{ (i,j),r}[\tau] 
%    \nonumber
%    \\ 
%    & + \sum_{r_2=1}^L \sum_{r_1=1}^L  {\bf G}^{\rm BS}_{r_2,\ell} {\bf \Phi}_{r_2}[\tau] {\bf G}^{\rm IRS}_{r_1,r_2} {\bf \Phi}_{r_1}[\tau] {\bf h}^{\rm IRS}_{ (i,j),r_1}[\tau] + ... \bigg),
%\end{align}
%where the IRS beamformers are set to ${\bf \Phi}_r[\tau] = {\rm diag}({\boldsymbol \phi}_{r}[\tau])$ $\forall r$.
%It is reasonable to assume that BS $\ell$ obtains the channels $\hat {\bf h}_{(i,j),\ell}[\tau] \; \forall i,j$ at time $\tau$ because pilot overhead for estimating the effective channels is negligible.
%To obtain SINR, BS $\ell$ applies the designed combiner ${\bf z}_{\ell, k}[\tau]$ to the received effective channels $\hat {\bf h}_{(i,j),\ell}[\tau] \; \forall i,j$ and obtains $\hat {\rm SINR}_{\ell, k}[\tau] $ as
%\begin{equation}
%    {\hat {\rm SINR}}_{\ell, k}[\tau] =
%{
%\frac{ |{\bf z}_{\ell, k}^H[\tau] \hat {\bf h}_{(\ell,k),\ell}[\tau]|^2 }
%{ \sum_{(i,j) \ne (\ell, k)} |{\bf z}_{\ell, k}^H[\tau] \hat {\bf h}_{(i,j),\ell}[\tau]|^2  + \sigma^2 }
%}.
%\end{equation}

%As above, BS $\ell$ can acquire the effective channels from all users, $\{ \hat {\bf h}_{(i,j),\ell}[\tau] \}_{i,j}$, and SINRs of the local users in cell $\ell$, $\{ {\hat {\rm SINR}}_{\ell, k}[\tau] \}_{k} $.



%In a typical system,
%the time-frequency resources are divided into physical resource blocks (PRBs) of coherence-time coherence-bandwidth product.
%Some resources (time slots or equivalently frequency channels) are used for channel estimation and the rest are used for data transmission.


%Each UE is allocated a set of PRBs over which UE sends pilot symbols.
%In an orthogonal frequency division multiplexing (OFDM) multi-access uplink network, we assume that each user receives allocation of a set of physical resource blocks (PRBs) for sending the pilot symbol.

%Then, the history is all previously-designed variables, $\{ {p}_{\ell,k}[\tau] \}_{\ell, k}$, $\{ {\bf z}_{\ell, k}[\tau] \}_{\ell, k}$, and $\{ {\boldsymbol \phi}_r[\tau] \}_r$ $\forall \tau < t$ , and the corresponding observations $\{ {\rm SINR}_{\ell, k}[\tau]\}_{\ell, k}$ and $\{ {\hat {\bf h}}_{(i, j),\ell}[\tau] \}_{i,j,\ell}$ $\forall \tau < t$.
%Therefore, to design the variables at current time slot $t$, $\{ {p}_{\ell, k}[t] \}_{\ell, k}$, $\{ {\bf z}_{\ell, k}[t] \}_{\ell, k} $, and $\{ {\boldsymbol \phi}_{r}[t] \}_{r}$,
%we can use the history of previous time $\forall \tau < t$. 


\subsection{Uplink Data Transmission Framework}


\begin{figure}[t]
  \includegraphics[width=\linewidth]{figures/timecrop.pdf}
  \centering
  \caption{Uplink data transmission framework for each BS.}
  \label{fig:timeline}
\end{figure}


As shown in Figure \ref{fig:timeline}, we design the framework of uplink data transmission.
Each coherence time $T$ is composed of two stages: Preparation and data transmission. The preparation stage consists of four phases: Uplink pilot transmission for local BS, information exchange between BSs, variables design of each BS and distribution to  UEs/IRS, and uplink pilot transmission for local/neighbouring BSs. We will focus on the cell $\ell$ (BS $\ell$) at time $t$. 

\subsubsection{Uplink pilot transmission for local BS}

Local BS $\ell$ receives the scalar effective channels from local UEs $(\ell,k)$ for $k \in \mathcal{K}$.
The UE $(l,k)$ transmits pilot symbol with the power $p_{\ell,k}[t-T]$ of previous time $t-T$ where IRS $r$ $\forall r \in \mathcal{L}$ were set to the beamforming vector ${\boldsymbol \phi}_{r}[t-T]$ of previous time $t-T$. 
This is because the uplink pilot transmission phase occurs before variables design. 
%This is one of strategy to measure the effect of channel variation with the same variables used.
Then, BS $\ell$ can obtain the scalar effective channels $\{ \tilde {h}_{(\ell,k),\ell,k'}[t] \}_{k,k' \in \mathcal{K}}$, which contain the outdated variables of time $t-T$ in it, which is given by
\begin{equation}
    \tilde {h}_{(\ell,k),\ell,k'}[t] = {\bf z}_{\ell, k'}^H[t-T] \tilde {\bf h}_{(\ell,k),\ell}[t],
\end{equation}
where $\tilde {\bf h}_{(\ell,k),\ell}[t] \in \mathbb{C}^{N_T \times 1}$ is the effective channel from UE $(\ell,k)$ to BS $\ell$, which has outdated UE powers and IRS beamformers in it, given by
\begin{multline}
    \tilde {\bf h}_{(\ell,k),\ell}[t] = \sqrt{p_{\ell,k}[t-T]} \bigg( {\bf h}^{\rm BS}_{ (\ell,k),\ell}[t]
    \\
    + \sum_{r=1}^L{\bf G}^{\rm BS}_{r,\ell} {\bf \Phi}_r[t-T] {\bf h}^{\rm IRS}_{ (\ell,k),r}[t] 
%    + \tilde {\bf g}^{\rm IRS }_{\ell}[t]
    \\+ \sum_{r_2=1}^L \sum_{r_1=1}^L  {\bf G}^{\rm BS}_{r_2,\ell} {\bf \Phi}_{r_2}[t-T] 
    {\bf G}^{\rm IRS}_{r_1,r_2} {\bf \Phi}_{r_1}[t-T] {\bf h}^{\rm IRS}_{ (\ell,k),r_1}[t]
    \bigg).
\end{multline}
%Note that $\tilde {\bf g}^{\rm IRS }_{\ell}[t]$ denotes the signals through multiple reflections between IRSs, which has outdated UE powers and IRS beamformers in it. The $\tilde {\bf g}^{\rm IRS }_{\ell}[t]$ can be formulated from \eqref{eq:multiIRSu} by replacing $p_{i,j}[t]$ with $p_{i,j}[t-T]$ and ${\boldsymbol \phi}_{r}[t]$ with ${\boldsymbol \phi}_{r}[t-T]$ for all $i \in \mathcal{L}, k \in \mathcal{K}, r \in \mathcal{L}$.



\subsubsection{Limitied information exchange}
We focus on BS $\ell$ receiving information from BS $i$ at time $t$.
The BS $\ell$ wants to receive information of UE $(\ell,k)$, such as the quantity how much UE $(\ell,k)$ decreased the performance of the data link of BS $i$. 
BS $\ell$ only receives information from BS $i$ in  neighbouring cell, where $i \in \mathcal{B}_{\ell, \rm to}[t]$. The $\mathcal{B}_{\ell, \rm to}[t]$ is the set of indices of neighbouring cells that are interfered by UEs in cell $\ell$, given by
\begin{multline}
    \mathcal{B}_{\ell, \rm to}[t] = \{ i \in \mathcal{L} : \sum_{k=1}^K \| \hat {\bf h}_{(\ell,k),i}[t] \|_2^2 \ge  \sum_{k=1}^K \| \hat {\bf h}_{(\ell,k),i'}[t] \|_2^2 ,
    \\ |\mathcal{B}_{\ell, \rm to}[t]|=N_N, i \in \mathcal{B}_{\ell, \rm to}[t], i' \in \mathcal{L}\backslash \mathcal{B}_{\ell, \rm to}[t]   \},
\end{multline}
BS $\ell $ selects the neighbouring cells 
based on the interferences by local UEs to other cell. Note that we consider $|\mathcal{B}_{\ell, \rm to}[t]|=N_N = 2$ in this paper. In large-scale networks with lots of cells, each BS only receives information from two cells.

In the information exchange phase at time $t$, BS $\ell$ can obtain the information of previous time $t-T$ from BS $i \in \mathcal{B}_{\ell, \rm to}[t-T]$. 
The exchanged information is the square of scalar effective channels, $\{ | \hat h_{(\ell,k),i,j} [t-T] |^2 \}_{k,j \in \mathcal{K}}$ and the sum-penalty value, $P_{\ell,i}[t-T]$. 
Here, $P_{\ell,i}[t-T]$ can be calculated at BS $i$ as
\begin{align}
    & P_{\ell,i}[t-T] = \sum_{j=1}^K P_{\ell,(i,j)}[t-T]
    \nonumber
    \\
    & = \sum_{j=1}^K \bigg[ \log_2 \bigg(1+ 
    \frac{ |\hat {h}_{(i,j),i,j}[t-T]|^2 }
    { \sum\limits_{(i',j') \ne (i,j),(\ell, \forall k) } |\hat {h}_{(i',j'),i,j}[t-T]|^2  + \sigma^2}
    \bigg) 
    \nonumber
    \\ & \quad\quad\quad - R_{i,j}[t-T]
     \bigg]
     \label{eq:penalty}
\end{align}
where $P_{\ell,(i,j)}[t-T]$ is the penalty value meaning the rate loss due to the UEs $(\ell, \forall k)$ in cell $\ell$ to the data rate of the UE $(i,j)$. 
The term with $\log_2(\cdot)$ denotes the data rate of UE $(i,j)$ without the interferences from UEs $(\ell, \forall k)$. This is the desirable data-rate of UE $(i,j)$ with respect to the interference of UEs $(\ell, \forall k)$. $R_{i,j}[t-T]$ is the data rate of UE $(i,j)$ including the interferences from UEs $(\ell, \forall k)$.
If the interference from UEs $(\ell, \forall k)$ is zero, then the two terms are equal, leading to the penalty term zero. On the other hand, if UEs $(\ell, \forall k)$ interferes with the data links of UE $(i,j)$, then the penalty is non-zero positive.

BS $i$ transfers the sum-penalty value to inform BS $\ell$ of how much performance is degraded due to UEs in cell $\ell$. This feedback information will enable for BS $\ell$, as an agent, to decrease the interferences to other cells by designing  variables in its own cell properly. For BS $\ell$, total number of exchanged information is $N_N(K^2+1)$. With $N_N=2$ and $K=3$, only 20 real values are exchanged for each cell.

%\begin{figure}[t]
%  \includegraphics[width=\linewidth]{figures/infoex.pdf}
%  \centering
%  \caption{Information exchange at time $t$. This figure demonstrates what types of information BS $\ell$ receives from BS $i$.}
%  \label{fig:infoex}
%\end{figure}


\subsubsection{Variables design and distribution to UEs/IRS}
\label{subsubsec:vardist}

From information exchange and local observations, BS $\ell$ collects sufficient information for multi-agent deep reinforcement learning. Then, BS $\ell$ will update its variables at time $t$, $\{ {p}_{\ell, k}[t] \}_{k}$, $\{ {\bf z}_{\ell, k}[t] \}_{k}$, and ${\boldsymbol \phi}_{\ell}[t] $, based on the proposed multi-agent deep Q-learning algorithm provided in Section \ref{subsec:MARL}. 

Once the variables are designed, BS $\ell$ distributes the information of the updated power  to UE $(\ell,k)$ for $k \in \mathcal{K}$ and the information of the updated IRS beamforming vector to IRS $\ell$.
The simple approach for variable distribution is that BS $\ell$ transfers the value of power ${p}_{\ell, k}[t]$ and the beamforming vector to IRS $\ell$.
It may be burdensome to transmit information every time $T$ to UEs and IRS, although BS transfers just the index to UEs/IRS. Considering low-rate wireless links between IRS and BS, we propose to use one-bit for transmission.
%The UE power are not drastically changing between consecutive times. Also, 
%However, this update requires lots of transmission overhead especially for IRS. 


%may be sometimes unrealistic because the power of UEs or element values (phase shifter) of IRS cannot change drastically between consecutive times. 

To reduce transmission overhead, BS $\ell$ transfers only one-bit to UEs and IRS at a time, where 1 or 0 denotes the sign of the gradient. 
Specifically, if BS $\ell$ transfers 1 to UE $(\ell,k)$ at time $t$, then UE $(\ell,k)$ increases the index number in the set of power values such that $i^{p}_{\ell,k}[t] = i^{p}_{\ell,k}[t-T] + 1 $, where $i^{p}_{\ell,k}[t-T]$ is the index corresponding to $p_{\ell,k}[t-T]$ in the set $\mathcal{P}$. since $\mathcal{P}$ is composed of increasing power values, the power is increased. 
If BS $\ell$ transfers 0, then UE $(\ell,k)$ decreases the index number in the set of power values such that $i^{p}_{\ell,k}[t] = i^{p}_{\ell,k}[t-T] - 1 $, leading to decreased power at time $t$.
%the power such that $p_{\ell,k}[t] = p_{\ell,k}[t-T] + \Delta_p $. If BS $\ell$ transfers 0, then UE decreases the power $p_{\ell,k}[t] = p_{\ell,k}[t-T] - \Delta_p $.
If BS $\ell$ transfers 1 to IRS $\ell$, then IRS $\ell$ increases the index number in the codebook such that $i^{\phi}_{\ell}[t] = i^{\phi}_{\ell}[t-T] + 1 $, where $i^{\phi}_{\ell}[t-T]$ is the index number corresponding to ${\boldsymbol \phi}_{\ell}[t-T]$ in the codebook $\mathcal{Q}$.
On the other hand, BS $\ell$ transfers 0 to IRS $\ell$, then $i^{\phi}_{\ell}[t] = i^{\phi}_{\ell}[t-T] - 1 $. This one-bit information update significantly reduces the transmission overhead from BS $\ell$ to IRS $\ell$,  and therefore is desirable in low-rate wireless link between BS and IRS.



%lets each user know how to update the power. For example, BS $\ell$ can transfer the value of power
%${p}_{\ell, k}[t]$ to UE $(\ell,k)$ for $k \in \mathcal{K}$ or transfer just single bit for the update direction such that 1 means increasing power and 0 means decreasing power.


\subsubsection{Uplink pilot transmission}
UE $(i,j)$ transmits pilot symbol with the updated power ${p}_{i,j}[t]$ where IRS $r$ $\forall r \in \mathcal{L}$ are set to the updated beamforming vector ${\boldsymbol \phi}_{r}[t]$.
Then, BS $\ell$ measures the scalar effective channel from local UEs $\{ \hat {h}_{(\ell,k),\ell,k'}[t]\}_{k,k' \in \mathcal{K}} $ and from UEs in neighbouring cells $\{ \hat {h}_{(i,j),\ell,k}[t]\}_{j,k \in \mathcal{K}, i \in \mathcal{B}_{\ell, \rm from}[t]} $.
%and  and neighbouring UEs for $(i,j) \in \mathcal{B}_\ell[t]$ with the combiner ${\bf z}_{\ell, k}[t]$.
%The obtained information obtained will be used as in the next time exchanged between BSs at next time $t+T$.
